Insights on Variance Estimation for Blocked and Matched Pairs Designs

Evaluating blocked randomized experiments from a potential outcomes perspective has two primary branches of work. The first focuses on larger blocks, with multiple treatment and control units in each block. The second focuses on matched pairs, with a single treatment and control unit in each block. These literatures not only provide different estimators for the standard errors of the estimated average impact, but they are also built on different sets of assumptions. Neither literature handles cases with blocks of varying size that contain singleton treatment or control units, a case which can occur in a variety of contexts, such as with different forms of matching or post-stratification. In this paper, we reconcile the literatures by carefully examining the performance of variance estimators under several different frameworks. We then use these insights to derive novel variance estimators for experiments containing blocks of different sizes.

==> blocking variance/blocking_variance_appendices.tex <==
%\documentclass[12pt]{article}
%\RequirePackage{amsmath,amssymb}
%
%\usepackage{amsthm}
%\usepackage[titletoc,title]{appendix}
%%\usepackage[toc,page]{appendix}
%\usepackage{array}
%\usepackage{bm}
%%\usepackage{cite}
%\usepackage{color}
%\usepackage{graphicx}
%\usepackage{epstopdf}
%\usepackage[letterpaper, portrait, margin=1in]{geometry}
%\usepackage{lipsum}
%\usepackage{listings}
%\usepackage{fancyref}
%\usepackage{float}
%\usepackage[font=footnotesize,labelfont=bf]{caption}
%\usepackage{xr}
%\externaldocument{blocking_variance}
%\usepackage{xcite}
%%\usepackage{chngcntr}
%%\usepackage{apptools}
%%\usepackage{thmtools, thm-restate}
%%\externalcitedocument{blocking_variance_pashley_miratrix}
%%\addbibresource{poststratref.bib}
%
%\usepackage{natbib}
%
%%\AtAppendix{\counterwithin{theorem}{section}}
%%\declaretheorem{theorem}
%\newtheorem{lemma}{Lemma}[subsection]
%\newtheorem{theorem}{Theorem}[subsection]
%\newtheorem{proposition}{Proposition}[subsection]
%\newtheorem{corollary}{Corollary}[subsection]
%
%\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
%\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
%\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
%
%
% 
%\theoremstyle{remark}
%\newtheorem*{remark}{Remark}
%
%%True treatment effects
%\newcommand*\taufs{\tau_{\mathcal{S}}}
%\newcommand*\taukfs{\tau_{k, \mathcal{S}}}
%\newcommand*\tauk{\tau_{k}}
%\newcommand*\tausbfs{\tau_{(SMALL),\mathcal{S}}}
%\newcommand*\tausbj{\tau_{(SMALL), j}}
%\newcommand*\tausbfsj{\tau_{(SMALL), \mathcal{S}, j}}
%\newcommand*\tausbfsone{\tau_{(SMALL), \mathcal{S}, 1}}
%\newcommand*\tausb{\tau_{(SMALL)}}
%\newcommand*\taubig{\tau_{(BIG)}}
%\newcommand*\taubigfs{\tau_{(BIG), \mathcal{S}}}
%\newcommand*\tauonejfs{\tau_{1, j, \mathcal{S}}}
%
%%Potential outcomes and means
%\newcommand*\poobs{Y_{i}^{obs}}
%\newcommand*\pot{Y_{i}(t)}
%\newcommand*\poc{Y_{i}(c)}
%\newcommand*\poz{Y_{i}(z)}
%\newcommand*\meanpot{\bar{Y}(t)}
%\newcommand*\meanpoc{\bar{Y}(c)}
%\newcommand*\meanpoz{\bar{Y}(z)}
%\newcommand*\meanpotk{\bar{Y}_k(t)}
%\newcommand*\meanpock{\bar{Y}_k(c)}
%\newcommand*\meanpozk{\bar{Y}_k(z)}
%\newcommand*\meanpotobs{\bar{Y}^{obs}(t)}
%\newcommand*\meanpocobs{\bar{Y}^{obs}(c)}
%\newcommand*\meanpozobs{\bar{Y}^{obs}(z)}
%\newcommand*\meanpotkobs{\bar{Y}_k^{obs}(t)}
%\newcommand*\meanpockobs{\bar{Y}_k^{obs}(c)}
%\newcommand*\meanpozkobs{\bar{Y}_k^{obs}(z)}
%\newcommand*\popmeanpoz{\mu(z)}
%\newcommand*\popmeanpot{\mu(t)}
%\newcommand*\popmeanpoc{\mu(c)}
%\newcommand*\popmeanpozk{\mu_k(z)}
%\newcommand*\popmeanpotk{\mu_k(t)}
%\newcommand*\popmeanpock{\mu_k(c)}
%
%
%%Model symbol
%\newcommand*\model{\mathcal{F}}
%
%%Expectation
%\newcommand*\EE{\mathbb{E}}
%
%%Count symbols
%\newcommand*\nk{n_k}
%\newcommand*\nck{n_{c, k}}
%\newcommand*\ntk{n_{t, k}}
%\newcommand*\nzk{n_{z, k}}
%\newcommand*\numsbunits{n_{sb}}
%\newcommand*\numsizej{m_{j}}
%\newcommand*\numsb{K_{j}}
%
%%Treatment effect estimators
%\newcommand*\tauestbk{\widehat{\tau}_{(BK)}}
%\newcommand*\tauestcr{\widehat{\tau}_{(CR)}}
%\newcommand*\taukest{\widehat{\tau}_{k}}
%\newcommand*\tausbest{\widehat{\tau}_{(SMALL)}}
%\newcommand*\taubigest{\widehat{\tau}_{(BIG)}}
%\newcommand*\tausbjest{\widehat{\tau}_{(SMALL), j}}
%\newcommand*\tausbmest{\widehat{\tau}_{(SMALL/m)}}
%\newcommand*\tausbinfest{\widehat{\tau}_{(SMALL), inf}}
%\newcommand*\tauonejest{\widehat{\tau}_{1, j}}
%\newcommand*\tauonejfsest{\widehat{\tau}_{1, j, fs}}
%
%%Sample variances
%\newcommand*\Sc{S^{2}(c)}
%\newcommand*\St{S^{2}(t)}
%\newcommand*\Sz{S^2(z)}
%\newcommand*\Stc{S^{2}(tc)}
%\newcommand*\scest{s^{2}(c)}
%\newcommand*\stest{s^{2}(t)}
%\newcommand*\szest{s^{2}(z)}
%\newcommand*\scplg{\tilde{s}^{2}(c)}
%\newcommand*\stplg{\tilde{s}^{2}(t)}
%\newcommand*\szplg{\tilde{s}^{2}(z)}
%\newcommand*\stcest{s^{2}(tc)}
%\newcommand*\Sck{S^{2}_k(c)}
%\newcommand*\Stk{S^{2}_k(t)}
%\newcommand*\Szk{S^{2}_k(z)}
%\newcommand*\Stck{S^{2}_k(tc)}
%\newcommand*\sckest{s^{2}_k(c)}
%\newcommand*\stkest{s^{2}_k(t)}
%\newcommand*\szkest{s^{2}_k(z)}
%\newcommand*\stckest{s^{2}_k(tc)}
%\newcommand*\sckplg{\tilde{s}^{2}_k(c)}
%\newcommand*\stkplg{\tilde{s}^{2}_k(t)}
%\newcommand*\szkplg{\tilde{s}^{2}_k(z)}
%
%%Population variances 
%\newcommand*\sigmac{\sigma^{2}(c)}
%\newcommand*\sigmat{\sigma^{2}(t)}
%\newcommand*\sigmaz{\sigma^{2}(z)}
%\newcommand*\sigmatc{\sigma^{2}(tc)}
%\newcommand*\sigmack{\sigma^{2}_k(c)}
%\newcommand*\sigmatk{\sigma^{2}_k(t)}
%\newcommand*\sigmazk{\sigma^{2}_k(z)}
%\newcommand*\sigmatck{\sigma^{2}_k(tc)}
%
%
%%Variance estimators
%\newcommand*\varestcr{\widehat{\sigma}^{2}_{(CR)}}
%\newcommand*\varestk{\widehat{\sigma}^{2}_{k}}
%\newcommand*\varestbkone{\widehat{\sigma}^{2}_{(BK)}}
%\newcommand*\varestbktwo{\widehat{\sigma}^{2}_{(BK), 2}}
%\newcommand*\varestbkthree{\widehat{\sigma}^{2}_{(BK), 3}}
%\newcommand*\varestsb{\widehat{\sigma}^{2}_{(SMALL)}}
%\newcommand*\varestsbone{\widehat{\sigma}^{2}_{(SMALL), 1}}
%\newcommand*\varestsbm{\widehat{\sigma}^{2}_{(SMALL/m)}}
%\newcommand*\varestsbp{\widehat{\sigma}^{2}_{(SMALL/p)}}
%\newcommand*\varestsbs{\widehat{\sigma}^{2}_{(SMALL/s)}}
%\newcommand*\varestsbj{\widehat{\sigma}^{2}_{(SMALL), j}}
%\newcommand*\varestsbinf{\widehat{\sigma}^{2}_{(SMALL), inf}}
%\newcommand*\varestplg{\widehat{\sigma}^{2}_{(PLG)}}
%
%
%% Editing macros
%\usepackage{color}
%
%\newcommand\cmnt[2]{\qquad{{\color{red} \em #1---#2} \qquad}}
%\newcommand\cmntM[1]{\cmnt{#1}{Miratrix}}
%\newcommand\awk{{{\color{red} {$\leftarrow$ Awkward phrasing}}\qquad}}
%\newcommand\cmntMp[1]{{\color{red} $\leftarrow$ {\em #1 -Miratrix} \qquad}}
%
%%Label figures with S for supplementary
%\renewcommand{\thefigure}{S\arabic{figure}}
%\renewcommand{\theequation}{S\arabic{equation}}
%
%\begin{document}
%\appendix
%\setcounter{page}{1}
\begin{center}
{\bf \Large  Supplementary Material\\for\\``Insights on Variance Estimation for Blocked and Matched Pairs Designs''}

\vspace{0.5cm}
{ \large Nicole E. Pashley and Luke W. Miratrix}
\end{center}



\medskip 


These Supplementary Material primarily contain detailed derivations of the results in the main paper, as well as some additional results and discussion. 
We first give some detail on the notational elements in the main paper. We then proceed with a non-technical discussion of alternate estimators for variance estimation.
We next provide additional results and further details on simulations.
We finally give derivations for the results in the main paper.
More detailed proofs for some of these sections are available upon request. 




\addcontentsline{toc}{section}{Introduction}


\section{Alternative strategies for variance estimation}\label{append:var_est_alt}
In the main paper we examined strategies for variance estimation that put no structure on how the individual blocks may differ from each other.
At root, the focus is on estimating the residual variance of units around their block means, and aggregating appropriately.

This section discusses alternatives along with when they might be more or less appropriate.
The first two subsections describe estimators that require model assumptions.
These estimators may perform well in certain circumstances (i.e., those where the model assumptions hold), but rely on assumptions that we do not make in our analysis.
They can therefore perform very poorly under misspecification.
The third subsection describes an estimator used for matched pairs that is proposed in the RCT-YES software documentation.
This RCT-YES estimator assumes a specific population model that we do not consider in our paper.

\subsection{Linear regression}\label{subsubsec:var_est_lin_reg}
Perhaps the most common method of estimation for randomized trials is to simply fit a linear model to the data with a treatment indicator and a dummy variable for each block.
If there is no interaction between the treatment and block dummies, this approach will produce a precision-weighted estimate of the treatment effect, with an overall implicit estimand of a weighted average of the average impacts within each block, weighted by the estimated block precision under a homoscedasticity assumption.
If there is impact variation correlated with this precision, then this precision-weighted estimand could be different than the overall ATE, resulting in a biased estimator.
Furthermore, if blocks have different proportions of treated units and different sizes, this weighting might not correspond to any easily interpretable quantity.
As pointed out by \citeauthor{freedman_2008b}, this regression model is also not justified by randomization, which results in complications with the corresponding standard errors (\citeauthor{freedman_2008a},~2008a,b).
Unfortunately, however, this approach is likely the most common in the field.

The above issues are, in part, repairable. 
\cite{winston_lin} shows that the estimator from a linear model including interactions between the treatment indicator and block dummies is unbiased.
In fact, this estimator is equivalent to the blocked estimator presented in this paper.
The question is then how to estimate the standard errors from within the ordinary least squares framework.
Lin advocates a Huber-White sandwich estimator for the general covariate case, but these have problems when the blocks have single treated or single control units.
In particular, several variants of these estimators, such as HC2 and HC3, will not even be defined due to the characteristics of the corresponding design matrix.
The HC0 estimator can still be heavily biased if there is systematic heteroscedasticity across the blocks.
\cite{gerber_green_text} (p. 116-117) advocate a weighted estimator, but this can also fail in the presence of blocks with singleton treated or control units.

\subsection{Pooling variance estimates}\label{subsec:var_est_plg}
As we have seen, the driving idea behind the big block estimator to get an overall variance is to obtain variance estimates for all of the block specific estimates, and then combine them in a weighted average.
This does not work for small blocks, as we do not have enough units to estimate variances of one of the treatment arms.
If we had such estimates, however, we could aggregate as before.

One way forward is to use the variance estimates in other blocks to estimate the variances in the intractable blocks.
For example, if treatment effects within block were considered constant, one could use the variance estimate of the larger of the treatment or control group of the block as the variance of the other treatment arm.
Alternatively, if given a means of assessing how similar blocks are in terms of their variance, one could simply use the variance of the closest big block for each small block.
This typically requires some assumptions that, based on covariate values of the blocks, the variances of the potential outcomes are the same or similar.
Similarly, Abadie and Imbens created an estimator of the variance for matched pairs that involves pairing the closest matched pairs and creating a pooled variance estimator for the two blocks together \citep[][]{abadie2008}.
They found that their estimator was asymptotically unbiased given certain conditions, such as the closeness of pairs increasing as the sample size grew.
Although the asymptotic results derived in their paper are not necessarily appropriate here, this could be a reasonable plug-in estimator under the assumptions that (i) the covariate(s) that create the strata are related to the potential outcomes and variance and that (ii) the small strata are more similar to each other than the larger strata.

Covariates could also be exploited using linear regression to predict variance for the intractable blocks or estimate a variance model for all blocks in a pooled manner; see, for example, \cite{fogarty_2017}.
If we believe that the variance of the estimator in each block is related to the block size, we could fit a linear regression for the big blocks, of variance versus their size, and then extrapolate to the small blocks.
Alternatively, if nothing is known and there are very few small blocks, an average (or the largest) of the big block variance estimates might be used.

Any of these plug-in estimators can either be used for all the blocks or used to simply fill in any missing components of the small blocks.
For instance, if all of the small blocks are such that they have multiple controls but only one treated unit, we can calculate $\sckest$ as usual but approximate $\stkest$ based on one of the previously mentioned methods.

In general, many plug-ins could be appropriate, based on what assumptions the researcher is able to make.
The choice of plug-in estimator should be chosen prior to running the experiment and should be based on the researchers assumptions and knowledge at that time.
Trying several plug-in estimators and using the smallest will create bias. 

\subsection{The RCT-YES estimator}\label{subsubsec:rct_yes_est}
One might also consider an estimator suggested in the RCT-YES manuscript \citep[][p. 83]{schochet_2016}.
The form of this estimator, using block sizes as weights, is
\[\widehat{\sigma}^2_{RCT} = \frac{1}{K\left(K-1\right)(\frac{n}{K})^2}\sum_{k=1}^K\left(n_k\taukest - \frac{n}{K}\tauestbk\right)^2 . \]
As discussed and proven in the RCT-YES documentation, this estimator is consistent under an infinite population of an infinite number of strata of infinite size, where we sample strata and then units within strata.
This is the random sampling of strata setting in the remark of Section~\ref{subsec:inf_finstrat_framework}.
This estimator differs from our estimators $\varestsbm$ and $\varestsbp$ by putting the weights inside the square.
Unfortunately, moving the weighting inside the squares can cause large bias in the finite setting and the stratified sampling framework.
In fact, in the simulations comparing variance estimator performance in the finite sample, presented in Section~\ref{sec:sim}, the RCT-YES bias and variance was high enough that it was not comparable to the other estimators presented.
This estimator is targeting a superpopulation quantity, thus the standard errors are larger in part to capture the additional variation of the strata being a random sample.

We discussed the performance of the original RCT-YES estimator with Dr. Schochet (personal correspondence, April 2018), and he proposed an alternate estimator.
Again using the block sizes as weights, this estimator has the form
\[\widehat{\sigma}^2_{RCT, 2} = \frac{1}{K\left(K-1\right)(\frac{n}{K})^2}\sum_{k=1}^K\nk^2\left(\taukest - \tauestbk\right)^2 \]
and is rooted in survey sampling methods \citep{CochranWilliamG.WilliamGemmell1977St}.
This estimator is more stable because the weights are not inside the parentheses.
This estimator is still motivated by a superpopulation sampling framework, and takes the variability of the blocks into account.
Finite sample performance using this estimator on all of the blocks does not perform well, unless all blocks have the same $\tau_k$, which aligns with what we expect from explorations of our small block estimators.
If used in combination as a hybrid estimator, its performance is very similar to that of the hybrid using $\varestsbp$.

\section{Connecting to \cite{mukerjee2018using}}\label{supp:muk_et_al_paper}

\cite{mukerjee2018using} sets up a framework for representing conservative variance estimators for a very general set of causal estimands and estimators.
The big block variance estimator, $\varestbkone$, falls within their framework, as shown in their paper.
We can also show that the small block estimators $\varestsbs$ and $\varestsbm$ do as well.
However, it does not seem that our other small block estimator, $\varestsbp$, is within their framework scope.
In fact, it appears necessary to go beyond this framework, as we have done with $\varestsbp$, to obtain a conservative variance estimator for small blocks of variable size when there are not multiple blocks of the same size.
Note that the hybrid estimator corresponding to any small block estimator that can be obtained within their framework can also be obtained within their framework.
We present some details below to understand these connections more clearly.

Under the notation of \cite{mukerjee2018using}, they consider $T$ to be any partition of units into treatment groups.
In other words, it represents a single assignment of units into treatment and control.
As all of the partitions $T$ are equally probably under the block randomized assignment mechanism and it is clear that we are focusing on block randomization here, we will largely drop this notation.
We next define quantities used in \cite{mukerjee2018using} but not in our paper, but largely keep with the notation from our paper.
Equation (5) of \cite{mukerjee2018using} defines the treatment effect estimator as 
\[\widehat{\tau} = \sum_{z \in \{c,t\}}g(z)\widehat{\bar{Y}}(z), \]
where $\widehat{\bar{Y}}(z)$ is some sort of average of units under treatment $z$ and in our case $g(t) = 1$ and $g(c) = -1$.
Equation (6) defines 
\[\widehat{\bar{Y}}(z) = a(T,z) + \sum_{i: Z_i=z}b_i(T,z)Y_i(z).\]
In our case $a(T,z) = 0$ and $b_i(T,z) = \frac{\nk}{n}\frac{1}{\nzk}$ for units in block $k$ under treatment $z$ such that
\[\widehat{\bar{Y}}(z)=\sum_{k=1}^K\sum_{i: Z_i=z, b_i=k} \frac{\nk}{n}\frac{1}{\nzk}Y_i(z) = \sum_{k=1}^K \frac{\nk}{n}\meanpozkobs.\]
Then we have
\[\widehat{\tau}=\tauestbk=\sum_{k=1}^K \frac{\nk}{n}\left(\meanpotkobs-\meanpockobs\right),\]
as desired.

To layout the framework for variance estimation of \cite{mukerjee2018using}, we need to define some more quantities.
First, we have the probabilities
\begin{align*}
\pi_i(z) &= E[\mathbb{I}_{Z_i=z}] = \frac{\nzk}{\nk} \quad \text{for unit $i: b_i=k$,}\\
\pi_{ii^*}(z, z^*) &= E[\mathbb{I}_{Z_i=z}\mathbb{I}_{Z_{i^*}=z^*}] = \begin{cases}
\frac{\nzk}{\nk}\frac{n_{z^*,j}}{n_j} & \text{for unit $i : b_i=k$, $i^*: b_{i^*}=j$ with $k \neq j$,}\\
\frac{\nzk(\nzk-1)}{\nk(\nk-1)} & \text{for unit $i, i^*: b_i=b_{i^*} = k$, $z = z^*$,}\\
\frac{\ntk\nck}{\nk(\nk-1)} & \text{for unit $i, i^* : b_i=b_{i^*} = k$, $z \neq z^*$.}\\
\end{cases}
\end{align*}

Then we have the quantities from equations (12) of \cite{mukerjee2018using}, which we simplify in our setting as follows:
\begin{align*}
M &= \sum_{z\in \{c,t\}} \sum_{z^* \in \{c,t\}} g(z) g(z^*) A(z,z^*)\\
& = \sum_{z\in \{c,t\}} \sum_{z^* \in \{c,t\}} g(z) g(z^*) a(T,z)a(T,z^*)\\
& = 0,\\
M_i(z) &= g(z) \sum_{z^* \in \{c,t\}}  g(z^*) \left(A_i^{(1)}(z,z^*) + A_i^{(2)}(z^*,z)\right)\\
& = g(z) \sum_{z^* \in \{c,t\}}  g(z^*) \left(E[\mathbb{I}_{Z_i=z}]a(T,z^*)b_i(T,z) + E[\mathbb{I}_{Z_i=z^*}]a(T,z)b_i(T,z^*)\right)\\
& = 0,\\
M_{ii}(z) &= (g(z))^2B_{ii}(z, z)\\
& = (g(z))^2E[\mathbb{I}_{Z_i=z}(b_i(T,z))^2]\\
& = \frac{\nzk}{\nk}\left(\frac{\nk}{n}\frac{1}{\nzk}\right)^2 \quad \text{( for $i: b_i = k$)}\\
& = \frac{1}{n^2}\frac{\nk}{\nzk},\\
M_{ii^*}(z, z^*) &= g(z)g(z^*)B_{ii^*}(z, z^*)\\
&= g(z)g(z^*)E[\mathbb{I}_{Z_i=z}\mathbb{I}_{Z_{i^*}=z^*}b_i(T,z)b_{i^*}(T,z^*)]\\
& = \begin{cases}
g(z)g(z^*)\frac{1}{n^2} & \text{for unit $i: b_i=k$, $i^*: b_{i^*} = j$ with $k \neq j$,}\\
\frac{1}{n^2}\frac{\nk(\nzk-1)}{\nzk(\nk-1)} & \text{for unit $i, i^*: b_i = b_{i^*} = k$, $z = z^*$,}\\
-\frac{1}{n^2}\frac{\nk}{\nk-1} & \text{for unit $i, i^* : b_i = b_{i^*} = k$, $z \neq z^*$.}
\end{cases}
\end{align*}

To get the variance and variance estimators we need an additional quantity from Equation (17) of \cite{mukerjee2018using},
\begin{align*}
\tilde{M}_{ii^*}(z, z^*) &= g(z)g(z^*)\left[B_{ii^*}(z, z^*) + q_{ii^*} - \frac{1}{n^2}\right]\\
&=\begin{cases}
g(z)g(z^*)q_{ii^*} & \text{for unit $i: b_i=k$, $i^*: b_{i^*} = j$ with $k \neq j$,}\\
q_{ii^*} -\frac{1}{n^2}\frac{\nk-\nzk}{\nzk(\nk-1)}   & \text{for unit $i, i^*: b_i=b_{i^*} = k$, $z = z^*$,}\\
- \left[\frac{1}{n^2}\frac{1}{\nk-1} + q_{ii^*}\right]& \text{for unit $i, i^*:b_i = b_{i^*} = k$, $z \neq z^*$,}\\
\end{cases}
\end{align*}
with $q_{ii^*}$ being entries from a matrix, as explained below.

We can use these quantities to derive the true variance of the blocking estimator.
This was shown in \cite{mukerjee2018using} as an example of the use of their framework.
Further, those authors show that the variance can be written using some positive-semi definite $\bm{Q}$ matrix with $(i,i^*)$ entry denoted $q_{ii^*}$ such that $\bm{Q}\bm{J} = \bm{0}$, where $\bm{J}$ is a matrix of all ones, and $q_{ii} = 1/N^2$ (see equation (15), (18), (19) of \cite{mukerjee2018using}), as 
\[\text{var}(\widehat{\tau}) = V_{\bm{Q}}(\widehat{\tau}) - \bm{\tau}'\bm{Q}\bm{\tau},\]
where $\bm{\tau}' = (\tau_1,\dots,\tau_n)$ and
\begin{align*}
V_{\bm{Q}}(\widehat{\tau}) =& M + \sum_{z \in \{c,t\}}\sum_{i=1}^n\left(M_i(z)Y_i(z) + M_{ii}(z)(Y_i(z))^2\right)\\
&+\sum_{z \in \{c,t\}}\sum_{z^* \in \{c,t\}}\sum_{i=1}^n\sum_{i^* (\neq i) =1}^n\tilde{M}_{ii^*}(z,z^*)Y_i(z)Y_{i^*}(z^*).
\end{align*}
In our setting,
\begin{align*}
V_{\bm{Q}}(\tauestbk)=& \sum_{z \in \{c,t\}}\sum_{k=1}^K\sum_{i: b_i = k}\frac{1}{n^2}\frac{\nk}{\nzk}(Y_i(z))^2\\
&+ \sum_{z \in \{c,t\}}\sum_{k=1}^K\sum_{i: b_i=k}\sum_{i^*(\neq i): b_{i^*}=k} \left(q_{ii^*} -\frac{1}{n^2}\frac{\nk-\nzk}{\nzk(\nk-1)}\right)Y_i(z)Y_{i^*}(z)\\
& - 2\sum_{k=1}^K\sum_{i: b_i=k}\sum_{i^*(\neq i): b_{i^*}=k}\left(\frac{1}{n^2}\frac{1}{\nk-1} + q_{ii^*}\right)Y_i(t)Y_{i^*}(c)\\
&+\sum_{z \in \{c,t\}}\sum_{z^* \in \{c,t\}}\sum_{k=1}^K\sum_{j (\neq k)=1}^K\sum_{i:b_i=k}\sum_{i^*:b_{i^*}=j}g(z)g(z^*)q_{ii^*}Y_i(z)Y_{i^*}(z^*).
\end{align*}

Armed with this set up, the authors show that we can obtain a conservative variance estimator by estimating $V_{\bm{Q}}(\widehat{\tau})$ with (equation (21) of \cite{mukerjee2018using}),
\begin{align*}
\widehat{V}_{\bm{Q}}(\widehat{\tau}) =& M + \sum_{z\in \{c,t\}}\sum_{i:Z_i=z}\frac{1}{\pi_i(z)}\left(M_i(z)Y_i(z) + M_{ii}(z)(Y_i(z))^2\right)\\
& + \sum_{z\in \{c,t\}}\sum_{z^*\in \{c,t\}}\sum_{i: Z_i=z}\sum_{i^*(\neq i): Z_{i^*} = z^*}\frac{\tilde{M}_{ii^*}(z,z^*)}{\pi_{ii^*}(z,z^*)}Y_i(z)Y_{i^*}(z^*).
\end{align*}

In our setting, this simplifies to
\begin{align*}
\widehat{V}_{\bm{Q}}(\tauestbk)
=& \sum_{z\in \{c,t\}}\sum_{i: Z_i=z}\frac{M_{ii}(z)}{\pi_i(z)}(Y_i(z))^2 + \sum_{z\in \{c,t\}}\sum_{k=1}^K\sum_{i: b_i=k, Z_i=z}\sum_{i^*(\neq i): b_{i^*} =k, Z_{i^*}=z}\frac{\tilde{M}_{ii^*}(z,z)}{\pi_{ii^*}(z,z)}Y_i(z)Y_{i^*}(z)\\
& + 2\sum_{k=1}^K\sum_{i: b_i=k, Z_i=t}\sum_{i^*(\neq i): b_{i^*}=k, Z_{i^*}=c}\frac{\tilde{M}_{ii^*}(t,c)}{\pi_{ii^*}(t,c)}Y_i(t)Y_{i^*}(c)\\
& + \sum_{z\in \{c,t\}}\sum_{z^*\in \{c,t\}}\sum_{k=1}^K\sum_{j (\neq k)=1}^K\sum_{i: b_i=k, Z_i=z}\sum_{i^*: b_{i^*}=j, Z_{i^*}=z^*}\frac{\tilde{M}_{ii^*}(z,z^*)}{\pi_{ii^*}(z,z^*)}Y_i(z)Y_{i^*}(z^*)\\
%%
=& \underbrace{\sum_{z\in \{c,t\}}\sum_{k=1}^K\sum_{i: b_i=k, Z_i=z}\frac{\nk^2}{n^2}\frac{1}{\nzk^2}(Y_i(z))^2}_{\textbf{A}}\\
& +\underbrace{ \sum_{z\in \{c,t\}}\sum_{k=1}^K\sum_{i: b_i=k, Z_i=z}\sum_{i^*(\neq i): b_{i^*}=k, Z_{i^*}=z}\frac{q_{ii^*} -\frac{1}{n^2}\frac{\nk-\nzk}{\nzk(\nk-1)}}{\frac{\nzk(\nzk-1)}{\nk(\nk-1)}}Y_i(z)Y_{i^*}(z)}_{\textbf{B}}\\
& - \underbrace{2\sum_{k=1}^K\sum_{i: b_i=k, Z_i=t}\sum_{i^*: b_{i^*}=k, Z_{i^*}=c}\frac{\frac{1}{n^2}\frac{1}{\nk-1} + q_{ii^*}}{\frac{\ntk\nck}{\nk(\nk-1)}}Y_i(t)Y_{i^*}(c)}_{\textbf{C}}\\
& + \underbrace{\sum_{z\in \{c,t\}}\sum_{z^*\in \{c,t\}}\sum_{k=1}^K\sum_{j(\neq k)=1}^K\sum_{i: b_i=k, Z_i=z}\sum_{i^*: b_{i^*}=j, Z_{i^*}=z^*}\frac{g(z)g(z^*)q_{ii^*}}{\frac{\nzk}{\nk}\frac{n_{z^*,j}}{n_j}}Y_i(z)Y_{i^*}(z^*)}_{\textbf{D}}.
\end{align*}
To connect this type of estimator to the estimators in our paper, we need to find specifications of the $\bm{Q}$ matrix such that the estimators are equivalent.
In particular, according to the assumption in Equation (22) of \cite{mukerjee2018using}, this estimator requires $\pi_{ii^*}(z, z^*) >0$ whenever $\tilde{M}_{ii^*}(z,z^*) \neq 0$.
To meet this requirement, we need $\tilde{M}_{ii^*}(z,z^*) = 0$ whenever $\pi_{ii^*}(z, z^*) =0$, which occurs in term \textbf{B} in the above expression if we have one treated (or one control) unit in block $k$.
This means that for any block $k$ with only one unit assigned to treatment $z$ we need
\[q_{ii^*} -\frac{1}{n^2}\frac{\nk-\nzk}{\nzk(\nk-1)} = 0  \implies q_{ii^*} =\frac{1}{n^2}\frac{\nk-\nzk}{\nzk(\nk-1)} = \frac{1}{n^2}\frac{\nk-1}{\nk-1} = \frac{1}{n^2}\]
for $i, i^*: b_i = b_{i^*} = k$.


To connect estimators of the form $\widehat{V}_{\bm{Q}}(\tauestbk)$ to our variance estimators for hybrid blocked experiments, we will put our small block estimators in the same form as  $\widehat{V}_{\bm{Q}}(\tauestbk)$ to make the comparison easier.
Our pooled small block estimator ($\varestsbp$), as well as the matched pairs estimator ($\varestsbs$), is of the following form, where $a_k$ are some weights such that $a_k-2\frac{\nk}{n}a_k + \frac{\nk^2}{n^2}\sum_{j=1}^Ka_j = \nk^2/n^2$ (see Supplementary Material~\ref{append:var_est_small_p_derv} for proof that the weights for $\varestsbs$ and $\varestsbp$ have this property):
\begin{align*}
&\sum_{k=1}^Ka_k\left(\taukest - \tauestbk\right)^2\\
 &= \sum_{k=1}^Ka_k\left(\taukest^2 - 2\tauestbk\taukest+\tauestbk^2\right)\\
&= \sum_{k=1}^Ka_k\left(\taukest^2 - 2\frac{\nk}{n}\taukest^2 - 2\taukest\sum_{j\neq k}\frac{n_j}{n}\widehat{\tau}_{j}+\sum_{h=1}^K\frac{n_h^2}{n^2}\widehat{\tau}_{h}^2+\sum_{h=1}^K\sum_{f\neq h}\frac{n_hn_f}{n^2}\widehat{\tau}_{h}\widehat{\tau}_{f}\right)\\
&= \sum_{k=1}^K\left(a_k-2\frac{\nk}{n}a_k + \frac{\nk^2}{n^2}\sum_{h=1}^Ka_h\right)\taukest^2 +\sum_{k=1}^K\sum_{j \neq k}\left(\frac{\nk n_j}{n^2}\sum_{h=1}^Ka_h - 2a_k\frac{n_j}{n}\right)\taukest\widehat{\tau}_{j}\\
&= \sum_{k=1}^K\left(\frac{\nk^2}{n^2}\right)\Bigg(\sum_{z \in \{c,t\}}\sum_{i: b_i=k, Z_i=z}\frac{1}{\nzk^2}\left(Y_i(z)\right)^2  +\sum_{z \in \{c,t\}}\sum_{i: b_i = k, Z_i=z}\sum_{i^* (\neq i): b_{i^*} = k, Z_{i^*}=z}\frac{1}{\nzk^2}Y_i(z)Y_{i^*}(z)\\
& \qquad \qquad \qquad \qquad  -2\sum_{i:b_i=k, Z_i=t}\sum_{i^*: b_{i^*}=k, Z_{i^*}=c}\frac{1}{\ntk\nck}Y_i(t)Y_{i^*}(c)\Bigg)\\
& \quad+\sum_{k=1}^K\sum_{j \neq k}\left(\frac{\nk n_j}{n^2}\sum_{h=1}^Ka_h - 2a_k\frac{n_j}{n}\right)\sum_{z\in \{c,t\}}\sum_{z^*\in \{c,t\}}\sum_{i: b_i=k, Z_i=z}\sum_{i^*: b_{i^*}=j, Z_{i^*}=z^*}\frac{g(z)g(z^*)}{\nzk n_{z^*,j}}Y_i(z)Y_{i^*}(z^*)\\
&= \underbrace{\sum_{k=1}^K\frac{\nk^2}{n^2}\sum_{z \in \{c,t\}}\sum_{i:b_i=k, Z_i=z}\frac{1}{\nzk^2}\left(Y_i(z)\right)^2}_{\textbf{A}_1}+\underbrace{\sum_{k=1}^K\frac{\nk^2}{n^2}\sum_{z \in \{c,t\}}\sum_{i: b_i=k, Z_i=z}\sum_{i^* (\neq i):b_{i^*}=k, Z_{i^*}=z}\frac{1}{\nzk^2}Y_i(z)Y_{i^*}(z)}_{\textbf{B}_1}\\
&\quad -\underbrace{2\sum_{k=1}^K\frac{\nk^2}{n^2}\sum_{i: b_i=k, Z_i=t}\sum_{i^*: b_{i^*}=k, Z_{i^*}=c}\frac{1}{\ntk\nck}Y_i(t)Y_{i^*}(c)}_{\textbf{C}_1}\\
& \quad+\underbrace{\sum_{k=1}^K\sum_{j \neq k}\left(\frac{\nk n_j}{n^2}\sum_{h=1}^Ka_h - 2a_k\frac{n_j}{n}\right)\sum_{z\in \{c,t\}}\sum_{z^*\in \{c,t\}}\sum_{i: b_i=k, Z_i=z}\sum_{i^*: b_{i^*}=j, Z_{i^*}=z^*}\frac{g(z)g(z^*)}{\nzk n_{z^*,j}}Y_i(z)Y_{i^*}(z^*)}_{\textbf{D}_1}.\\
\end{align*}

We see that $\textbf{A}_1$ already matches $\textbf{A}$ from $\widehat{V}_{\bm{Q}}(\tauestbk)$.
We can simplify \textbf{B} and \textbf{C} using $q_{ii^*} = 1/n^2$ for $i, i^*$ in block $k$ such that there is only one unit assigned to $z$.


Starting with term $\textbf{B}$, note that if we assume each block is small (has one treated or one control) unit then for one $z$ term \textbf{B} is 0 and for the other we have, for units in block $k$, constant
\begin{align*}
\frac{q_{ii^*} -\frac{1}{n^2}\frac{\nk-\nzk}{\nzk(\nk-1)}}{\frac{\nzk(\nzk-1)}{\nk(\nk-1)}}&=\frac{\frac{1}{n^2} -\frac{1}{n^2}\frac{\nk-\nzk}{\nzk(\nk-1)}}{\frac{\nzk(\nzk-1)}{\nk(\nk-1)}}\\
&=\frac{1}{n^2}\frac{\nzk(\nk-1) -\nk+\nzk}{\frac{\nzk^2(\nzk-1)}{\nk}}\\
&=\frac{1}{n^2}\frac{\nk(\nzk-1)}{\frac{\nzk^2(\nzk-1)}{\nk}}\\
&=\frac{\nk^2}{n^2}\frac{1}{\nzk^2}.
\end{align*}
So we have that $\textbf{B}_1$ matches \textbf{B}.

Now for \textbf{C},
\begin{align*}
\frac{\frac{1}{n^2}\frac{1}{\nk-1} + q_{ii^*}}{\frac{\ntk\nck}{\nk(\nk-1)}} &= \frac{\frac{1}{n^2}\frac{1}{\nk-1} + \frac{1}{n^2}}{\frac{\ntk\nck}{\nk(\nk-1)}}\\
 &=\frac{1}{n^2} \frac{\frac{\nk}{\nk-1}}{\frac{\ntk\nck}{\nk(\nk-1)}}\\
  &=\frac{\nk^2}{n^2} \frac{1}{\ntk\nck}.
\end{align*}
Hence we have $\textbf{C}_1$ matches \textbf{C}.

Now we have the final term, in which we need to specify $q_{ii^*}$ for $i$ and $i^*$ in different blocks.
Let's start by simplifying the constant for $\textbf{D}_1$.
Now we will have to plug in the $a_k$ for $\varestsbp$.
\begin{align*}
\frac{\nk n_j}{n^2}\sum_{h=1}^Ka_h - 2a_k\frac{n_j}{n} =&\frac{\nk n_j}{n^2}\left(\sum_{h=1}^Ka_h - 2\frac{a_k}{\nk}n\right)\\
=&\frac{\nk n_j}{n^2}\left(\frac{\sum_{h=1}^K\frac{n_h^2}{n-2n_h}}{n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}} - \frac{2\nk n}{(n-2\nk)\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}\right)\\
=&\frac{\nk n_j}{n^2}\left(\frac{(n-2\nk)\sum_{h=1}^K\frac{n_h^2}{n-2n_h}-2\nk n}{(n-2\nk)\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}\right)\\
=&\frac{\nk n_j}{n^2}\left(\frac{n\sum_{h=1}^K\frac{n_h^2}{n-2n_h}-2\nk\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}{(n-2\nk)\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}\right)\\
=&\frac{\nk n_j}{n^2}\left(\frac{n\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)-n^2-2\nk\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}{(n-2\nk)\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}\right)\\
=&\frac{\nk n_j}{n^2}\left(1-\frac{n^2}{(n-2\nk)\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}\right)
\end{align*}
So, comparing to term \textbf{D}, we need
\[q_{ii^*} = \frac{1}{n^2}\left(1-\frac{n^2}{(n-2\nk)\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}\right).\]

First note that if all blocks are of the same size, R, in which case $\varestsbp$ reduces down to $\varestsbs$, then
\begin{align*}
\frac{1}{n^2}\left(1-\frac{n^2}{(n-2\nk)\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}\right) =&\frac{1}{R^2K^2}\left(1-\frac{R^2K^2}{(RK-2R)\left(RK+\sum_{h=1}^K\frac{R^2}{RK-2R}\right)}\right)\\
    =&\frac{1}{R^2K^2}\left(1-\frac{K}{K-1}\right)\\ 
    =&-\frac{1}{R^2K^2(K-1)}.
\end{align*}
This is actually essentially the same solution as example (b) in Section 5.1 of \cite{mukerjee2018using} for the split plot example with plots of the same size.
We can do a check that this works according to their criteria.
We need $\bm{Q}\bm{J} = \bm{0}$.
Let's take the $i$th row and arbitrary $j$th entry of $\bm{Q}\bm{J}$.
For all units belonging to the same block as unit $i$, $q_{ii^*} = 1/n^2$. Otherwise, $q_{ii^*} = 1/(n^2(K-1))$.
\begin{align*}
[\bm{Q}\bm{J}]_{ij} =& \frac{R}{n^2} - \frac{R(K-1)}{R^2K^2(K-1)}\\
=& \frac{R}{R^2K^2} - \frac{1}{RK^2}\\
=& 0
\end{align*}
So yes: for multiple blocks of the same size, the standard matched pairs variance estimator, $\varestsbs$, falls within the \cite{mukerjee2018using} framework for variance estimators.

This means that we can also do a block diagonalized version of this $\bm{Q}$ matrix to get our non-pooled small block estimator, $\varestsbm$, where we split blocks up by size first and then block diagonalize according to these splits.
More generally, estimators will be block diagonalized according to whether the pieces of the variance estimators include terms from multiple blocks.
For instance, with the big block part of the estimator, we would have all of the big blocks being separate block diagonals because we estimate variance within each block separately.
Similarly, for $\varestsbm$ because we estimate the variance within each small block group of the same size separately, we would block diagonalize according to block size for that piece.
On the other hand, if we had all blocks of the same size then there is no block diagonal because $\varestsbs$ uses all of the blocks together to estimate the overall variance.

Now what about $\varestsbp$ for small blocks of varying size?
The $q_{ii^*}$ terms for $i: b_i=k$ and $i^*: b_{i^*} = j$ with $k \neq j$ would be,
\[q_{ii^*} = \frac{1}{n^2}\left(1-\frac{n^2}{(n-2\nk)\left(n+\sum_{h=1}^K\frac{n_h^2}{n-2n_h}\right)}\right),\]
which are not guaranteed to be symmetric in this case (because of the $\nk$ term in the denominator).
So the $\bm{Q}$ matrix would not fall into \cite{mukerjee2018using} framework because it is not positive semi-definite.
Note that we assure positivity of bias for our estimator by requiring that $\nk < n/2$ for all blocks when using the pooled estimator.
Therefore, our estimator does not seem to fall within their framework and it appears to us that extending beyond their framework is necessary to solve the problem of small blocks of variable size.



\section{Data generating process for simulations}\label{append:more_sim}

The data generating process used for the simulations comparing the variance estimators gives us a single finite data set.
We then repeatedly randomize units to treatment, according to blocked randomization, to assess finite sample behavior.

The initial potential outcomes for the units in each block were drawn from a bivariate normal distribution, with the means and covariance matrix as follows (shown for a unit in block $k$):
\[\begin{pmatrix}
Y_i(0)\\
Y_i(1)
\end{pmatrix}\sim MVN\left(
\begin{pmatrix}
\alpha_k\\
\alpha_k + \beta_k
\end{pmatrix},\begin{pmatrix}
1 & \rho\\
\rho &1
\end{pmatrix}\right).
\]

The correlation of potential outcomes, $\rho$, was varied among 0, 0.5, and 1.
We controlled how differentiated the blocks were, and how heterogeneous the treatment effects across blocks were, by varying $\alpha_k$ and $\beta_k$.
We set $\alpha_k$ as $\alpha_k = \Phi^{-1}\left(1-\frac{k}{K+1}\right)a$. 
Similarly, $\beta_k = 5 + \Phi^{-1}\left(1-\frac{k}{k+1}\right)b$. 
The larger the $a$, the more the mean control potential outcomes for the blocks were spread apart.
The larger the $b$, the more heterogeneous the treatment impacts.
The parameters $a$ and $b$ were each varied among the values (0,0.1,0.3,0.5,0.8,1,1.5,2).
We keep the number and sizes of blocks fixed.
The blocks were ordered by size with the smallest block as block one.
As a consequence, the smaller blocks have both larger means under control and larger average treatment effects.

Simulations were run over assignment of units to treatments under a blocked design, which was done 5000 times for each combination of factors.
Before evaluating our overall results, we first checked that the simulation values agreed with the biases calculated for our variance estimators via the bias formulas in Section~\ref{subsec:var_est_perf_fin} of our paper.
They did.
Replication code showing this is available.



\section{Simulation investigating the variance of the variance estimators}\label{append:var_est_var}

In this auxiliary simulation we examine how the blocking variance estimators compare amongst themselves in terms of their own variance.
To assess this, we examine the variance of our variance estimators from our simulation study in Section~\ref{sec:sim} with the data generating process given in Section~\ref{append:more_sim}.

Results are on Figure~\ref{plot:var_var}.
We see that, in terms of variance, the estimators are generally comparable.
We expect more instability from estimators that utilize only information from the estimated average treatment effects, not from the variation of the individual units.
We see that the weighted regression estimator has the lowest variability.

\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{var_est_var.pdf}
\caption{Simulations to assess variance estimators' variance.
The x-axis shows the standard deviation of block average treatment effects.
Points show the average across the values of $\rho$ and the standard deviation of block average control potential outcomes in the simulation. (The trends for different $\rho$ were essentially the same.) FE stands for fixed effects.}
\label{plot:var_var}
\end{figure}




%%
%% Creation of small block variance estimator
%% 

\section{Creation and bias of $\varestsbm$}\label{append:var_est_small_m}

We first construct the variance estimator $\varestsbm$, and then derive the bias for this estimator for different frameworks.

\subsection{Creation of $\varestsbm$, Equation~(\ref{eq:var_est_sb_m})}\label{append:var_est_sb_m_derv}
To formally state the method described by Equation~(\ref{eq:var_est_sb_m}) from Section~\ref{subsec:var_est_small}, we first express our estimands and estimators in terms of weighted averages of estimates within collections of same-size blocks.
In the following, let there be $J$ unique block sizes in the sample. 
Let $\numsizej$ be the $j$th block size and let $\numsb$ be the number of blocks in the population of size $\numsizej$.
So then $n = \sum_{j=1}^J\numsizej\numsb$.
In particular, the sample average treatment effect for all units in blocks of size $\numsizej$ is
\[\tausbfsj = \frac{1}{\numsb}\sum_{k: \nk = \numsizej} \taukfs.\]
Let $N_j = \numsizej \numsb$ be the total number of units in the small blocks of size $\numsizej$.
Then the overall sample average treatment effect in terms of these $\tausbfsj$ is
\begin{equation}
\tausbfs = \frac{1}{\sum_{i=1}^J N_j}\sum_{j=1}^J N_j \tausbfsj. \label{eq:tau_small_j}	
\end{equation}
$\tausbfs$ is the same as $\taufs$ as before; we add the subscript ``small'' here to clarify the notation when we discuss hybrid experiments.
Note that these definitions are analogous for the infinite population, which are indicated by removing the $\mathcal{S}$ subscript.

The treatment effect estimators can be written in analogous form to the above.
We have unbiased estimators $\tausbjest = \frac{1}{\numsb}\sum_{k: \nk = \numsizej} \taukest$ for the average treatment effects in blocks of size $\numsizej$.
Simply plug them into Equation~\ref{eq:tau_small_j} to obtain an overall treatment effect estimator.

As discussed in Section~\ref{subsec:var_est_small}, within each piece $j$, use a variance estimator with the same form as Equation~\ref{eq:var_est_sb_same_size}:
\begin{align*}
\varestsbj  = \frac{1}{\numsb(\numsb-1)}\sum_{k: \nk = \numsizej} (\taukest - \tausbjest)^{2}
\end{align*}

Then combine to create an overall variance estimator:
\begin{align*}
\varestsbm = \frac{1}{\left(\sum_{j=1}^J N_j \right)^2}\sum_{j=1}^J N_j^2\varestsbj. 
\end{align*}


\subsection{Proof of Corollary~\ref{lemma:var_est_sb_m_fin_samp} (Bias under finite sample) and Corollary~\ref{lemma:bias_var_est_sb_m_strat_samp} (Bias under stratified sampling)}\label{append:bias_var_est_sb_m_strat_samp}

\begin{proof}
For this section assume that we are in the finite sample framework. 
The results for the stratified sampling from an infinite population framework follow directly by changing the expectations and notation.

First we will focus on $\varestsbj$ which is the variance estimator for $\tausbjest$. 
Note that
\begin{align*}
\text{var}\left(\tausbjest|\mathcal{S}\right) &= \text{var}\left(\frac{1}{\numsb}\sum_{k: \nk = \numsizej} \taukest\Big|\mathcal{S}\right)= \frac{1}{\numsb^2}\sum_{k: \nk = \numsizej}\text{var}\left( \taukest|\mathcal{S}\right).
\end{align*}

\begin{align*}
\EE&\left[\varestsbj|\mathcal{S}\right]\\
 &=\EE\left[ \frac{1}{\numsb(\numsb-1)}\sum_{k: \nk = \numsizej} (\taukest - \tausbjest)^{2}\Big|\mathcal{S}\right]\\
&=\frac{1}{\numsb(\numsb-1)}\EE\left[\sum_{k: \nk = \numsizej} \left(\taukest^2 -2\taukest\tausbjest+ \tausbjest^2\right)\Big|\mathcal{S}\right]\\
&=\frac{1}{\numsb(\numsb-1)}\left(\sum_{k: \nk = \numsizej}\left[\text{var}\left(\taukest|\mathcal{S}\right) + \taukfs^2\right] - \numsb\left[\text{var}\left(\tausbjest|\mathcal{S}\right) + \tausbfsj^2\right]\right)\\
&=\frac{1}{\numsb(\numsb-1)}\left(\sum_{k: \nk = \numsizej}\left[\frac{\numsb - 1}{\numsb}\text{var}\left(\taukest|\mathcal{S}\right) + \taukfs^2\right] - \numsb \tausbfsj\right)\\
&=\frac{1}{\numsb^2}\sum_{k: \nk = \numsizej}\text{var}\left(\taukest|\mathcal{S}\right) + \frac{1}{\numsb(\numsb-1)}\sum_{k: \nk = \numsizej}\left(\taukfs - \tausbfsj\right)^2\\
&=\text{var}\left(\tausbjest|\mathcal{S}\right) + \frac{1}{\numsb(\numsb-1)}\sum_{k: \nk = \numsizej}\left(\taukfs - \tausbfsj\right)^2.
\end{align*}

So the bias is
\[\EE\left[\varestsbj|\mathcal{S}\right] - \text{var}\left(\tausbjest|\mathcal{S}\right)=\frac{1}{\numsb(\numsb-1)}\sum_{k: \nk = \numsizej}\left(\taukfs - \tausbfsj\right)^2.\]

Now we move our attention to $\varestsbm$ which is a variance estimator for $\tausbest$.

We have
\begin{align*}
\text{var}\left(\tausbest|\mathcal{S}\right) &= \text{var}\left(\frac{1}{\sum_{i=1}^J m_iK_i}\sum_{j=1}^J\numsizej\numsb\tausbjest|\mathcal{S}\right)\\
&= \frac{1}{\left(\sum_{i=1}^J m_iK_i\right)^2}\sum_{j=1}^J\left(\numsizej\numsb\right)^2\text{var}\left(\tausbjest|\mathcal{S}\right).
\end{align*}
So then
\begin{align*}
\EE&\left[\varestsbm|\mathcal{S}\right]\\
&=\frac{1}{\left(\sum_{i=1}^J m_iK_i\right)^2}\sum_{j=1}^J\left(\numsizej\numsb\right)^2\EE\left[\varestsbj|\mathcal{S}\right]\\
&=\text{var}\left(\tausbest|\mathcal{S}\right) + \sum_{j=1}^J\frac{\numsizej^2\numsb}{\left(\sum_{i=1}^J m_iK_i\right)^2(\numsb-1)}\sum_{k: \nk = \numsizej}\left(\taukfs - \tausbfsj\right)^2.
\end{align*}

So the bias is
\[\EE\left[\varestsbm|\mathcal{S}\right] - \text{var}\left(\tausbest|\mathcal{S}\right) = \sum_{j=1}^J\frac{\numsizej^2\numsb}{\left(\sum_{i=1}^J m_iK_i\right)^2(\numsb-1)}\sum_{k: \nk = \numsizej}\left(\taukfs - \tausbfsj\right)^2.\]
\end{proof}

\subsection{Proof of Corollary~\ref{lem:rand_samp_strat_varsbm} (Bias under random sampling of strata, conditioning on block size)}\label{append:bias_var_est_sb_m_inf_strat}

\begin{proof}
Assume that we are in the random sampling of strata framework of Section~\ref{subsec:inf_finstrat_framework}.
We are focusing in on just the set of strata of size $m_j$.
We can either consider that there only exist strata of this size or we can imagine a sampling mechanism that draws these strata independently from strata of other sizes (e.g. stratified sampling by strata size), which is the same as conditioning on the number of strata of each size in the sample.
Also,
\begin{align*}
\text{var}\left(\tausbjest|\model_2\right) &= \EE\left[\text{var}\left(\tausbjest|\mathcal{S}\right)|\model_2\right] + \text{var}\left(\EE\left[\tausbjest|\mathcal{S}\right]|\model_2\right).
\end{align*}

From Appendix \ref{append:bias_var_est_sb_m_strat_samp}, we can see that
\begin{align*}
\EE&\left[\varestsbj|\mathcal{S}\right] &=\text{var}\left(\tausbjest|\mathcal{S}\right) + \frac{1}{\numsb(\numsb-1)}\sum_{k: \nk = \numsizej}\left(\taukfs - \tausbfsj\right)^2.
\end{align*}

From standard results from sampling theory (see \cite[Chapter~2]{lohr2010sampling}) we have
\[\EE\left[\frac{1}{\numsb(\numsb-1)}\sum_{k: \nk = \numsizej}\left(\taukfs - \tausbfsj\right)^2|\model_2\right] = \frac{\sigma^2_\tau}{K_j} = \text{var}\left(\tausbjest|\model_2\right).\]

Hence, we end up with
\begin{align*}
\EE\left[\varestsbj|\model_2\right] &=\EE\left[\text{var}\left(\tausbjest|\mathcal{S}\right)|\model_2\right] + \text{var}\left(\EE\left[\tausbjest|\mathcal{S}\right]|\model_2\right).
\end{align*}

Thus, this is an unbiased variance estimator in this setting.

If we have varying size but condition on the number of strata of each size that we sample, then we use the fact that stratified sampling causes the estimators for each strata size to be independent.

The proof of this result for an infinite number of infinite size strata is direct by replacing the conditioning on $\mathcal{S}$ by conditioning on $\bm{B}$ and using results from the stratified sampling framework.
\end{proof}

\section{Creation and bias of $\varestsbp$}\label{append:var_est_small_p_derv}

We next construct the variance estimator $\varestsbp$ that can estimate variance across a heterogeneous assortment of blocks, and then derive its bias under different frameworks.



\subsection{Proof of Theorem~\ref{lemma:var_est_sb_p_fin_samp} (Bias under finite sample) and Corollary~\ref{lemma:bias_var_est_sb_p_strat_samp} (Bias under stratified sampling)}\label{append:var_est_small_p_proofs}
\begin{proof}
For this section assume that we are in the finite sample framework.
The results for the stratified sampling framework follow directly by changing what we are taking the expectation with respect to and exchanging notation.
We explain how $\varestsbp$  was derived which also provides the bias of the estimator in these two frameworks.

To begin we consider, for an experiment with all small blocks, a variance estimator of the form
\[ X \equiv \sum_{k=1}^K a_k \left(\taukest - \tauestbk\right)^2 \]
for some collection of $a_k$.
We then wish to find non-negative $a_k$'s that would make this estimator as close to unbiased as possible.
In particular, we aim to create an estimator with similar bias to $\varestsbm$ but that allows for blocks of varying size.
That is, we are looking to create a similarly conservative estimator that is unbiased when the average treatment effect is constant across blocks.
This also means that we are creating the minimally biased conservative estimator of this form, without further assumptions.

The expected value of an estimator of this form is
 \begin{align*}
 \EE&\left[ X |\mathcal{S}\right]\\
  =&   \EE\left[\sum_{k=1}^{K}a_{k}\left(\taukest - \taukfs + \taukfs - \taufs + \taufs - \tauestbk\right)^{2}|\mathcal{S}\right]\\
 =&   \EE\Big[\sum_{k=1}^{K}a_{k}\Big(\left(\taukest - \taukfs\right)^{2} + \left(\taukfs - \taufs\right)^{2} + \left(\taufs - \tauestbk\right)^{2}\\
 &+ 2\left(\taukest - \taukfs\right)\left(\taukfs - \taufs\right) + 2\left(\taukest - \taukfs\right)\left(\taufs - \tauestbk\right) + 2\left(\taukfs - \taufs\right)\left(\taufs - \tauestbk\right)\Big)|\mathcal{S}\Big]\\
 =&  \sum_{k=1}^{K}a_{k}\left(\text{var}\left(\taukest|\mathcal{S}\right) +  \EE\left[\left(\taukfs \!-\! \taufs\right)^{2}|\mathcal{S}\right] +  \underbrace{\EE\left[\left(\taufs\! -\! \tauestbk\right)^{2}|\mathcal{S}\right]}_{\textbf{A}} + 2 \underbrace{\EE\left[\left(\taukest \! - \! \taukfs\right)\left(\taufs \!-\! \tauestbk\right)|\mathcal{S}\right]}_{\textbf{B}}\right)
 \end{align*}
 

For \textbf{A}: 
  \begin{align*}
 \EE\left[(\taufs - \tauestbk)^{2}|\mathcal{S}\right] &=  \text{var}\left(\tauestbk|\mathcal{S}\right)=\sum_{k=1}^{K}\frac{\nk^{2}}{n^{2}}\text{var}\left(\taukest|\mathcal{S}\right)
 \end{align*}
 
 For \textbf{B}:
 \begin{align*}
 \EE\left[(\taukest - \taukfs)(\taufs - \tauestbk)|\mathcal{S}\right] &= \EE\left[\left(\taukest - \taukfs\right)\sum_{j=1}^{K}\frac{n_{j}}{n}\left(\tau_{j, \mathcal{S}} - \widehat{\tau}_{j}\right)\Big|\mathcal{S}\right]\\
 &= \EE\left[-\frac{\nk}{n}\left(\taukest - \taukfs\right)^{2} +\left(\taukest - \taukfs\right)\sum_{j \neq k}\frac{n_{j}}{n}\left(\tau_{j, \mathcal{S}} - \widehat{\tau}_{j, \mathcal{S}}\right)\Big|\mathcal{S}\right]\\
  &=-\frac{\nk}{n}\text{var}\left(\taukest|\mathcal{S}\right)
 \end{align*}

Due to the assignment mechanism, $\widehat{\tau}_{j}$ will be independent of $\widehat{\tau}_{k}$ so the cross terms are all zero in the above equation.
 
 Putting \textbf{A} and \textbf{B} together, we get
  \begin{align*}
\EE\left[X |\mathcal{S}\right] &= \sum_{k=1}^{K}a_{k}\text{var}\left(\taukest|\mathcal{S}\right) + \sum_{k=1}^{K}a_{k}\left(\taukfs - \taufs\right)^{2} + \sum_{k=1}^{K}a_{k}\sum_{j=1}^{K}\frac{n_{j}^{2}}{n^{2}}\text{var}\left(\widehat{\tau}_{j}|\mathcal{S}\right)\\
& \qquad - 2\sum_{k=1}^{K}a_{k}\frac{\nk}{n}\text{var}\left(\taukest|\mathcal{S}\right)\\
 &=  \sum_{k=1}^{K}\left(a_{k} - 2a_{k}\frac{\nk}{n} + \frac{n_{k}^{2}}{n^{2}}\sum_{j=1}^{K}a_{j}\right)\text{var}\left(\taukest|\mathcal{S}\right) + \sum_{k=1}^{K}a_{k}\left(\taukfs - \taufs\right)^{2}
 \end{align*}

We now select $a_k$ to make the above as close to the true variance as possible.
The second term will be small if the $\taukfs$ do not vary much.
But this is unknown and thus we cannot select universal $a_k$ to control it.
We would like
 \[a_{k} - 2a_{k}\frac{n_{k}}{n} + \frac{n_{k}^{2}}{n^{2}}\sum_{j=1}^{K}a_{j} = \frac{n_{k}^{2}}{n^{2}}\]
 so that the first term is the true variance.
Then the second term, the bias, would be similar to that of the standard matched pairs variance estimator.
 
If we solve the $a_{k}$ as above we will obtain a conservative estimator that is unbiased when we have equal average treatment effect for all blocks, for the stratified sampling or finite framework.
To show this, consider the bias:
 \begin{align}
 \EE\left[X|\mathcal{S}\right] &- \text{var}\left(\tauestbk|\mathcal{S}\right)\nonumber\\
  &=  \sum_{k=1}^{K}\left(a_{k} - 2a_{k}\frac{\nk}{n} + \frac{\nk^{2}}{n^{2}}\sum_{j=1}^{K}a_{j} - \frac{\nk^2}{n^2}\right)\text{var}\left(\taukest|\mathcal{S}\right) + \sum_{k=1}^{K}a_{k}\left(\taukfs - \taufs\right)^{2}.\label{eq:ex_var_sp}
 \end{align}

We know $\text{var}\left(\taukest|\mathcal{S}\right) \geq 0$ for all $k$.
We also have $\sum_{k=1}^{K}a_{k}\left(\taukfs - \taufs\right)^{2} \geq 0$ so at a minimum it is 0.
This implies that to always be conservative, the first term in the above expression must always be at least 0.
Hence, to minimize the bias but remain conservative, we set $a_{k} - 2a_{k}\frac{\nk}{n} + \frac{\nk^{2}}{n^{2}}\sum_{j=1}^{K}a_{j} - \frac{\nk^2}{n^2} = 0$.
Note that $\taukfs$ and $\taufs$ are unknown and so we cannot optimize with respect to them.
 
 
Denote $C = \sum_{k=1}^{K}a_{k}$.
 Then we want to solve
 
 \begin{align*}
 a_k - 2a_k\frac{\nk}{n} + \frac{\nk^2}{n^2}C &= \frac{\nk^2}{n^2}\\
 a_k(1 - 2\frac{\nk}{n}) &= \frac{\nk^2}{n^2}(1-C)\\
 a_k &= \frac{\nk^2}{n}\frac{1-C}{n - 2\nk}
 \end{align*}
 
 But then
 \begin{align*}
 C&= \sum_{k=1}^{K} a_k = \sum_{k=1}^{K} \frac{\nk^2(1-C)}{n(n-2\nk)}\\
 \left(1 + \frac{1}{n}\sum_{k=1}^{K} \frac{\nk^2}{n-2\nk}\right)C &= \frac{1}{n}\sum_{k=1}^{K} \frac{\nk^2}{n-2\nk}
 \end{align*}
 \begin{align*}
 C&=\frac{1}{n}\sum_{k=1}^{K}\frac{\nk^2}{n-2\nk}\left(\frac{1}{1+ \frac{1}{n}\sum_{j=1}^{K}\frac{n_j^2}{n-2n_j}}\right)
 = \frac{\sum_{k=1}^{K}\frac{\nk^2}{n-2\nk}}{n+\sum_{j=1}^{K}\frac{n_j^2}{n-2n_j}}
 \end{align*}
 
 Then we have
 \begin{align*}
 a_k &= \frac{\nk^2}{n}\left(\frac{1-C}{n - 2\nk}\right)
 = \frac{\nk^2}{(n-2\nk)(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}.
 \end{align*}
 
 So then 
 \[\sum_{k=1}^{K} \frac{\nk^2}{\left(n-2\nk\right)\left(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j}\right)}\left(\taukest - \tauestbk\right)^{2}\]
  has bias 
  \[\sum_{k=1}^{K} \frac{\nk^2}{\left(n-2\nk\right)\left(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j}\right)}\left(\taukfs - \taufs\right)^{2}.\]
Bigger strata get weighted more heavily.

As a check, in the case where the $n_k$ are all the same, so that $n = K\nk$, the above boils down to $a_k = \frac{1}{K(K-1)}$ and $C = \frac{1}{K-1}$, giving us the classic matched pairs variance estimator.
\end{proof}

\subsection{Proof of Theorem~\ref{theorem:var_sbp_rand_samp} (Unbiasedness of $\varestsbp$ given independence of block sizes and effects)}\label{append:varsbp_rand_samp}
\begin{proof}
We start from the Equation~\ref{eq:ex_var_sp}.
As in Section~\ref{append:var_est_small_p_derv}, let 
\[ X \equiv \sum_{k=1}^K a_k \left(\taukest - \tauestbk\right)^2. \]
Then
 \begin{align*}
 \EE\left[X|\mathcal{S}\right]
  &=  \sum_{k=1}^{K}\left(a_{k} - 2a_{k}\frac{\nk}{n} + \frac{\nk^{2}}{n^{2}}\sum_{j=1}^{K}a_{j}\right)\text{var}\left(\taukest|\mathcal{S}\right) + \sum_{k=1}^{K}a_{k}\left(\taukfs - \taufs\right)^{2}.
 \end{align*}
 
 Previously we were concerned with getting the first term correct.
 But in the Random Sampling of Strata setting, the second term is trickier.
 This is especially the case if we have large blocks and thus can estimate the first term.
 So first we focus on the second term.
 Keeping the variance decomposition in mind, we ultimately want the expectation of this second term to look like $\text{var}(\taufs)$.
 

 As a reminder, the variance decomposition is
 \begin{align*}
 \text{var}(\tauestbk|\model_2) &=\EE\left[\text{var}(\tauestbk|\mathcal{S})|\model_2\right]+\text{var}\left(\EE[\tauestbk|\mathcal{S}]|\model_2\right)\\
 &=\EE\left[\text{var}(\tauestbk|\mathcal{S})|\model_2\right]+\text{var}\left(\taufs|\model_2\right).\\
 \end{align*}

 
 We assume, for simplicity, that the block sizes are independent from the treatment effects.
 This implies that $\EE[\taukfs|\model_2] = \tau$.
 
 The expected value of the second term in this setting is
 \begin{align*}
 \EE&\left[ \sum_{k=1}^{K}a_{k}\left(\taukfs - \taufs\right)^{2}\Big|\model_2 \right]\\
    =& \EE\left[ \sum_{k=1}^{K}a_{k}\taukfs^2 -2\taufs\sum_{k=1}^{K}a_k\taukfs +\taufs^2\sum_{k=1}^{K}a_{k}\Big|\model_2\right]\\
    =& \EE\Bigg[ \sum_{k=1}^{K}a_{k}\taukfs^2 -2\left(\sum_{k=1}^{K}a_k\frac{\nk}{n}\taukfs^2 +\sum_{k=1}^K\sum_{j\neq k}a_k\frac{n_j}{n}\taukfs\tau_{j,\mathcal{S}}\right)\\
    &+\left(\sum_{k=1}^{K}\frac{\nk^2}{n^2}\taukfs^2 +\sum_{k=1}^K\sum_{j\neq k}\frac{\nk n_j}{n^2}\taukfs\tau_{j,\mathcal{S}}\right)\sum_{k=1}^{K}a_{k}\Big|\model_2\Bigg]\\
        =& \EE\left[ \sum_{k=1}^{K}\left(a_{k}-2a_k\frac{\nk}{n}+\frac{\nk^2}{n^2}\sum_{i=1}^{K}a_{i}\right)\taukfs^2 -\sum_{k=1}^K\sum_{j\neq k}\left(2a_k\frac{n_j}{n}-\frac{\nk n_j}{n^2}\sum_{i=1}^{K}a_{i}\right)\taukfs\tau_{j,\mathcal{S}}\Big|\model_2\right]\\
        =& \EE\left[ \sum_{k=1}^{K}\left(a_{k}-2a_k\frac{\nk}{n}+\frac{\nk^2}{n^2}\sum_{i=1}^{K}a_{i}\right)\taukfs^2\Big|\model_2\right] -\EE\left[ \sum_{k=1}^K\sum_{j\neq k}\left(2a_k\frac{n_j}{n}-\frac{\nk n_j}{n^2}\sum_{i=1}^{K}a_{i}\right)\Big|\model_2\right]\tau^2.\\
 \end{align*}
 
 Now consider the true variance, which we are trying to estimate.
 
 \begin{align*}
 \text{var}(\taufs|\model_2)&= \text{var}\left(\sum_{k=1}^K\frac{\nk}{n}\taukfs\Big|\model_2\right)\\
 &=\EE\left[\left(\sum_{k=1}^K\frac{\nk}{n}\taukfs - \tau\right)^2\Big|\model_2\right]\\
 &=\EE\left[\left(\sum_{k=1}^K\frac{\nk}{n}\taukfs\right)^2\Big|\model_2\right] - \tau^2\\
  &=\EE\left[\sum_{k=1}^K\frac{\nk^2}{n^2}\taukfs^2\Big|\model_2\right]+\EE\left[\sum_{k=1}^K\sum_{j\neq k}\frac{\nk n_j}{n^2}\taukfs\tau_{j,\mathcal{S}}\Big|\model_2\right] - \tau^2\\
    &=\EE\left[\sum_{k=1}^K\frac{\nk^2}{n^2}\taukfs^2\Big|\model_2\right]-\EE\left[\sum_{k=1}^K\frac{\nk^2}{n^2}\Big|\model_2\right]\tau^2
 \end{align*}
 
We have the last equality because
\begin{align*}
\EE\left[\sum_{k=1}^K\sum_{j\neq k}\frac{\nk n_j}{n^2}\taukfs\tau_{j,\mathcal{S}}\Big|\model_2\right] &= \EE\left[\sum_{k=1}^K\sum_{j\neq k}\frac{\nk n_j}{n}\Big|\model_2\right]\tau^2\\
&=\EE\left[\sum_{k=1}^K\frac{\nk}{n}(1-\frac{\nk}{n})\Big|\model_2\right]\tau^2 \\
&= \EE\left[1-\sum_{k=1}^K\frac{\nk^2}{n^2}\Big|\model_2\right]\tau^2.
\end{align*}


Matching this up with the expectation of our estimator, we want
\begin{align*}
\frac{\nk^2}{n^2}=a_{k}-2a_k\frac{\nk}{n}+\frac{\nk^2}{n^2}\sum_{i=1}^{K}a_{i}
\end{align*}

 and
 \begin{align*}
 \sum_{k=1}^K\frac{\nk^2}{n^2} = \sum_{k=1}^K\sum_{j\neq k}\left(2a_k\frac{n_j}{n}-\frac{\nk n_j}{n^2}\sum_{i=1}^{K}a_{i}\right).
 \end{align*}
 
 The first equation we solved for before in Section~\ref{append:var_est_small_p_derv}.
So we will get
 \[a_k = \frac{\nk^2}{(n-2\nk)(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}.\]

Let's see if this weight works for the second term.

\begin{align*}
&\sum_{k=1}^K\sum_{j\neq k}\left(2a_k\frac{n_j}{n}-\frac{\nk n_j}{n^2}\sum_{i=1}^{K}a_{i}\right)\\
&=\sum_{k=1}^K2a_k(1-\frac{\nk}{n})-(1-\sum_{k=1}^K\frac{\nk^2}{n^2})\sum_{i=1}^{K}a_{i}\\
&=\sum_{k=1}^K \frac{2\nk^2(1-\frac{\nk}{n})}{(n-2\nk)(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}-(1-\sum_{k=1}^K\frac{\nk^2}{n^2})\sum_{i=1}^{K} \frac{n_i^2}{(n-2n_i)(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}\\
%Trial
&=\sum_{k=1}^K \frac{\nk^2(1-2\frac{\nk}{n})}{(n-2\nk)(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}+\sum_{k=1}^K\frac{\nk^2}{n^2}\sum_{i=1}^{K} \frac{n_i^2}{(n-2n_i)(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}\\
&=\sum_{k=1}^K \frac{\nk^2(n-2\nk)}{n(n-2\nk)(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}+\sum_{k=1}^K\frac{\nk^2}{n^2}\sum_{i=1}^{K} \frac{n_i^2}{(n-2n_i)(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}\\
&=\sum_{k=1}^K \frac{\nk^2}{n(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}+\sum_{k=1}^K\frac{\nk^2}{n^2}\sum_{i=1}^{K} \frac{n_i^2}{(n-2n_i)(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}\\
&=\sum_{k=1}^K\frac{\nk^2(n+\sum_{i=1}^K \frac{n_i^2}{(n-2n_i)})}{n^2(n+\sum_{j=1}^K\frac{n_j^2}{n-2n_j})}\\
&=\sum_{k=1}^K\frac{\nk^2}{n^2}
\end{align*}

Which is exactly what we wanted.
So this weight works.
And because it is the same as the weight for the finite sample (where we wanted to get the first term in the variance decomposition correct), this also takes care of the first term in the variance decomposition.

The proof of this result for an infinite number of infinite size strata is direct by replacing the conditioning on $\mathcal{S}$ by conditioning on $\bm{B}$ and using results from the stratified sampling framework.
 \end{proof}
 
 
 
 \section{Creation of $\widehat{\sigma}^2_{SRS}$, Equation~(\ref{eq:var_est_srs_bk})}\label{append_var_srs}

In this section we derive a variance estimator for the case of simple random sampling and flexible blocks.
This framework includes the case of units coming from a simple random sample, with the blocks made after the fact.

We begin with the basic variance decomposition to examine what we are trying to estimate.
Let $\sigmatc$ be the population variance of treatment effects.

\begin{align}
 \text{var}(\tauestbk|SRS) &=\EE\left[\text{var}(\tauestbk|\mathcal{S})|SRS\right]+\text{var}\left(\EE[\tauestbk|\mathcal{S}]|SRS\right)\nonumber\\
 &=\EE\left[\sum_{k=1}^K\frac{\nk^2}{n^2}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}-\frac{\Stck}{\nk}\right)\Big|SRS\right]+\text{var}\left(\taufs|SRS\right)\nonumber\\
  &=\EE\left[\sum_{k=1}^K\frac{\nk^2}{n^2}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}-\frac{\Stck}{\nk}\right)\Big|SRS\right]+\frac{\sigmatc}{n}\nonumber\\
  &=\EE\left[\sum_{k=1}^K\frac{\nk^2}{n^2}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}-\frac{\Stck}{\nk}\right)\Big|SRS\right]+\EE\left[\frac{\Stc}{n}\Big|SRS\right] \nonumber\\
    &=\underbrace{\EE\left[\sum_{k=1}^K\frac{\nk^2}{n^2}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}\right)\Big|SRS\right]}_{\textbf{A}}+\underbrace{\EE\left[\frac{\Stc}{n}-\sum_{k=1}^K\frac{\nk}{n}\frac{\Stck}{n}\Big|SRS\right]}_{\textbf{B}}\label{eq_srs_breakdown}
\end{align}

Let's examine $\Stc$ so we can simplify term \textbf{B}.
\begin{align*}
\Stc &= \sum_{k=1}^K\frac{\nk-1}{n-1}\Stck + \sum_{k=1}^K\frac{\nk}{n-1}\left(\taukfs-\taufs\right)^2
\end{align*}

So term \textbf{B} can simplify as follows:
\begin{align*}
\Stc-\sum_{k=1}^K\frac{\nk}{n}\Stck &=\sum_{k=1}^K\frac{\nk-1}{n-1}\Stck + \sum_{k=1}^K\frac{\nk}{n-1}\left(\taukfs-\taufs\right)^2 -\sum_{k=1}^K\frac{\nk}{n}\Stck\\
&=\sum_{k=1}^K\frac{\nk}{n-1}\left(\taukfs-\taufs\right)^2 -\sum_{k=1}^K\frac{n-\nk}{n(n-1)}\Stck.
\end{align*}

Now recall from Supplementary Materials~\ref{append:var_est_small_p_derv} that
  \begin{align*}
\EE\left[\sum_{k=1}^K a_k \left(\taukest - \tauestbk\right)^2 |\mathcal{S}\right] 
 &=  \sum_{k=1}^{K}\left(a_{k} - 2a_{k}\frac{\nk}{n} + \frac{n_{k}^{2}}{n^{2}}\sum_{j=1}^{K}a_{j}\right)\text{var}\left(\taukest|\mathcal{S}\right) + \sum_{k=1}^{K}a_{k}\left(\taukfs - \taufs\right)^{2}.
 \end{align*}
 
 Letting $a_k = \nk$, we have
   \begin{align*}
\EE&\left[\sum_{k=1}^K \nk \left(\taukest - \tauestbk\right)^2 \Big|\mathcal{S}\right]\\
 &=  \sum_{k=1}^{K}\left(\nk - \frac{\nk^2}{n}\right)\text{var}\left(\taukest|\mathcal{S}\right) + \sum_{k=1}^{K}\nk\left(\taukfs - \taufs\right)^{2}\\
  &=  \sum_{k=1}^{K}\frac{\nk(n-\nk)}{n}\text{var}\left(\taukest|\mathcal{S}\right) + \sum_{k=1}^{K}\nk\left(\taukfs - \taufs\right)^{2}\\
    &=  \sum_{k=1}^{K}\frac{\nk(n-\nk)}{n}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}-\frac{\Stck}{\nk}\right) + \sum_{k=1}^{K}\nk\left(\taukfs - \taufs\right)^{2}\\
  &=  \sum_{k=1}^{K}\frac{\nk(n-\nk)}{n}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}\right) + \sum_{k=1}^{K}\nk\left(\taukfs - \taufs\right)^{2} -\sum_{k=1}^{K}\frac{(n-\nk)}{n}\Stck\\
    &=  \sum_{k=1}^{K}\frac{\nk(n-\nk)}{n}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}\right) + (n-1)\left(\Stc-\sum_{k=1}^K\frac{\nk}{n}\Stck\right).
 \end{align*}
 
 This means that
    \begin{align*}
\EE&\left[\sum_{k=1}^K \frac{\nk}{n(n-1)} \left(\taukest - \tauestbk\right)^2 \Big|\mathcal{S}\right]
 =\sum_{k=1}^{K}\frac{\nk(n-\nk)}{n^2(n-1)}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}\right) + \frac{\Stc}{n}-\sum_{k=1}^K\frac{\nk}{n}\frac{\Stck}{n}.
 \end{align*}
 
 So we have a way to estimate term \textbf{B} of Equation~\ref{eq_srs_breakdown}, which means we just need to add in a correction to get term \textbf{A}.
 \begin{align*}
& \sum_{k=1}^{K}\frac{\nk^2}{n^2}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}\right)-\sum_{k=1}^{K}\frac{\nk(n-\nk)}{n^2(n-1)}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}\right)\\
 &= \sum_{k=1}^{K}\frac{\nk(\nk-1)}{n(n-1)}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}\right)
 \end{align*}
 
 Putting it all together, we have
 \begin{align*}
\EE\left[ \sum_{k=1}^{K}\frac{\nk(\nk-1)}{n(n-1)}\left(\frac{\Sck}{\nck}+\frac{\Stk}{\ntk}\right) + \sum_{k=1}^K \frac{\nk}{n(n-1)} \left(\taukest - \tauestbk\right)^2\Big|SRS\right]= \text{var}(\tauestbk|SRS).
 \end{align*}
 
 So 
 \[\widehat{\sigma}^2_{SRS} = \sum_{k=1}^{K}\frac{\nk(\nk-1)}{n(n-1)}\left(\frac{\sckest}{\nck}+\frac{\stkest}{\ntk}\right) + \sum_{k=1}^K \frac{\nk}{n(n-1)} \left(\taukest - \tauestbk\right)^2\]
 is an unbiased variance estimator.




%\bibliographystyle{apalike}
%\bibliography{poststratref}{}


%\end{document}





